Diffuse interstellar bands in the HII region M17: Insights into their relation with the total-to-selective visual extinction $R_V$

Diffuse interstellar bands (DIBs) are broad absorption features measured in sightlines probing the diffuse interstellar medium. Although large carbon-bearing molecules have been proposed as the carriers producing DIBs, their identity remains unknown. The sight line to the young massive star-forming region M17 shows anomalous extinction in the sense that the total-to-selective extinction parameter differs significantly from the average Galactic value and may reach values $R_{V} > 4$. Given the high $R_V$ values, we investigate whether the DIBs in sight lines towards young OB stars in M17 show a peculiar behaviour. We measure the properties of the most prominent DIBs in M17 and study these as a function of $E(B-V)$ and $R_{V}$. The DIB strengths in M17 concur with the observed relations between DIB equivalent width and reddening $E(B-V)$ in Galactic sight lines. For several DIBs we discover a linear relation between the normalised DIB strength EW/$A_{V}$ and $R_{V}^{-1}$. These trends suggest two groups: (i) a group of ten moderately strong DIBs that show a sensitivity to changes in $R_{V}$ that is modest and proportional to DIB strength, and (ii) a group of four very strong DIBs that react sensitively and to a similar degree to changes in $R_{V}$, but in a way that does not appear to depend on DIB strength. The DIB behaviour as a function of reddening is not peculiar in sight lines to M17. Also, we do not detect anomalous DIB profiles as seen in Her 36. DIBs are stronger, per unit visual extinction, in sight lines characterised by a smaller value of $R_{V}$ (large fraction of small dust particles). New relations between extinction normalised DIB strengths, EW/$A_V$, and $R_V$ support the idea that DIB carriers and interstellar dust are connected. Given the distinct behaviour of two groups of DIBs, different types of carriers do not necessarily relate to the dust grains in a similar way.

==> tables/Table_sideways.tex <==
\begin{sidewaystable}
\setlength{\tabcolsep}{3pt}
\centering 
 \caption{\normalsize\normalsize{DIB properties for lines-of-sight in M17. For each DIB the first column indicates the FHWM in nm and the second the EW and its error in m$\AA$.}}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
 \hline 
 \hline 
&    \multicolumn{2}{c|}{443.0}	&    \multicolumn{2}{c|}{578.12}	&    \multicolumn{2}{c|}{579.7}	&    \multicolumn{2}{c|}{619.62}	&    \multicolumn{2}{c|}{628.4}	&    \multicolumn{2}{c|}{637.9}	&    \multicolumn{2}{c|}{661.36}	&    \multicolumn{2}{c|}{862.0}	&    \multicolumn{2}{c|}{1179.7}	&    \multicolumn{2}{c|}{1317.6}	&    \multicolumn{2}{c|}{1526.8}	\\
 \hline 
	 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW		 & 	F 	 & 	 EW	\\
	 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$		 & 	nm 	 & 	 m$\AA$	\\
 \hline 
B111	 & 	1.9	 & 	$2027 \pm 8$	 & 	0.2	 & 	$558 \pm 6$	 & 	0.1	 & 	$91 \pm 6$	 & 	0.1	 & 	$60 \pm 6$	 & 	0.3	 & 	$1691 \pm 4$	 & 	0.1	 & 	$42 \pm 2$	 & 	0.1	 & 	$195 \pm 3$	 & 	0.5	 & 	$392 \pm 2$	 & 	0.3	 & 	$278 \pm 4$	 & 	0.6	 & 	$923 \pm 47$	 & 	$-$	 & 	$-$ 	\\
B164	 & 	2.1	 & 	$2539 \pm 44$	 & 	0.2	 & 	$513 \pm 12$	 & 	0.1	 & 	$143 \pm 26$	 & 	0.1	 & 	$62 \pm 13$	 & 	0.3	 & 	$1790 \pm 8$	 & 	0.1	 & 	$57 \pm 8$	 & 	0.1	 & 	$209 \pm 13$	 & 	0.5	 & 	$562 \pm 6$	 & 	0.3	 & 	$262 \pm 7$	 & 	0.6	 & 	$1134 \pm 18$	 & 	0.7	 & 	$875 \pm 2$ 	\\
B215	 & 	2.9	 & 	$4794 \pm 54$	 & 	0.2	 & 	$753 \pm 18$	 & 	0.2	 & 	$247 \pm 7$	 & 	0.1	 & 	$60 \pm 11$	 & 	0.4	 & 	$2206 \pm 9$	 & 	$-$	 & 	$-$	 & 	0.1	 & 	$259 \pm 5$	 & 	0.5	 & 	$471 \pm 5$	 & 	0.3	 & 	$205 \pm 7$	 & 	0.7	 & 	$1161 \pm 18$	 & 	0.6	 & 	$521 \pm 4$ 	\\
B243	 & 	1.7	 & 	$1779 \pm 66$	 & 	0.2	 & 	$515 \pm 26$	 & 	0.2	 & 	$283 \pm 10$	 & 	0.1	 & 	$58 \pm 15$	 & 	0.3	 & 	$1720 \pm 11$	 & 	$-$	 & 	$-$	 & 	0.1	 & 	$190 \pm 9$	 & 	0.5	 & 	$485 \pm 5$	 & 	0.4	 & 	$306 \pm 15$	 & 	0.7	 & 	$1115 \pm 60$	 & 	$-$	 & 	$-$ 	\\
B253	 & 	2.0	 & 	$2020 \pm 29$	 & 	0.2	 & 	$506 \pm 18$	 & 	0.1	 & 	$215 \pm 10$	 & 	0.1	 & 	$51 \pm 15$	 & 	0.3	 & 	$1708 \pm 12$	 & 	0.1	 & 	$42 \pm 8$	 & 	0.1	 & 	$179 \pm 6$	 & 	0.4	 & 	$370 \pm 5$	 & 	0.3	 & 	$269 \pm 12$	 & 	0.6	 & 	$1044 \pm 41$	 & 	0.7	 & 	$615 \pm 5$ 	\\
B268	 & 	1.9	 & 	$1742 \pm 31$	 & 	0.3	 & 	$649 \pm 21$	 & 	0.3	 & 	$229 \pm 16$	 & 	0.1	 & 	$55 \pm 15$	 & 	0.3	 & 	$1580 \pm 9$	 & 	0.1	 & 	$24 \pm 8$	 & 	0.1	 & 	$200 \pm 9$	 & 	0.5	 & 	$493 \pm 4$	 & 	0.4	 & 	$336 \pm 8$	 & 	0.6	 & 	$1016 \pm 43$	 & 	0.6	 & 	$820 \pm 2$ 	\\
B275	 & 	1.8	 & 	$1919 \pm 6$	 & 	0.2	 & 	$563 \pm 11$	 & 	0.2	 & 	$133 \pm 3$	 & 	0.1	 & 	$64 \pm 9$	 & 	0.3	 & 	$1661 \pm 11$	 & 	0.1	 & 	$39 \pm 7$	 & 	0.1	 & 	$209 \pm 13$	 & 	0.4	 & 	$400 \pm 5$	 & 	0.2	 & 	$173 \pm 9$	 & 	0.3	 & 	$463 \pm 15$	 & 	$-$	 & 	$-$ 	\\
B289	 & 	2.3	 & 	$3304 \pm 53$	 & 	0.2	 & 	$714 \pm 37$	 & 	0.1	 & 	$135 \pm 33$	 & 	0.1	 & 	$75 \pm 14$	 & 	0.4	 & 	$1920 \pm 18$	 & 	0.1	 & 	$62 \pm 14$	 & 	0.1	 & 	$239 \pm 12$	 & 	0.4	 & 	$457 \pm 7$	 & 	0.3	 & 	$255 \pm 7$	 & 	0.5	 & 	$928 \pm 22$	 & 	0.5	 & 	$438 \pm 3$ 	\\
B311	 & 	2.3	 & 	$2528 \pm 9$	 & 	0.2	 & 	$584 \pm 18$	 & 	0.2	 & 	$162 \pm 14$	 & 	0.1	 & 	$63 \pm 6$	 & 	0.3	 & 	$1770 \pm 8$	 & 	0.1	 & 	$76 \pm 6$	 & 	0.1	 & 	$228 \pm 5$	 & 	0.6	 & 	$506 \pm 2$	 & 	0.3	 & 	$261 \pm 5$	 & 	0.5	 & 	$859 \pm 29$	 & 	0.5	 & 	$401 \pm 4$ 	\\
B331	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	0.1	 & 	$386 \pm 39$	 & 	$-$	 & 	$-$	 & 	0.6	 & 	$318 \pm 10$	 & 	0.5	 & 	$796 \pm 35$	 & 	$-$	 & 	$-$ 	\\
B337	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	$-$	 & 	0.5	 & 	$630 \pm 8$	 & 	1.0	 & 	$457 \pm 21$	 & 	0.7	 & 	$1635 \pm 41$	 & 	$-$	 & 	$-$ 	\\
\hline 
\end{tabular}
\label{P3:tab:DIBs}
\end{sidewaystable} 

